Implicit Decomposition for Write-Efficient Connectivity Algorithms

The future of main memory appears to lie in the direction of new technologies that provide strong capacity-to-performance ratios, but have write operations that are much more expensive than reads in terms of latency, bandwidth, and energy. Motivated by this trend, we propose sequential and parallel algorithms to solve graph connectivity problems using significantly fewer writes than conventional algorithms. Our primary algorithmic tool is the construction of an $o(n)$-sized "implicit decomposition" of a bounded-degree graph $G$ on $n$ nodes, which combined with read-only access to $G$ enables fast answers to connectivity and biconnectivity queries on $G$. The construction breaks the linear-write "barrier", resulting in costs that are asymptotically lower than conventional algorithms while adding only a modest cost to querying time. For general non-sparse graphs on $m$ edges, we also provide the first $o(m)$ writes and $O(m)$ operations parallel algorithms for connectivity and biconnectivity. These algorithms provide insight into how applications can efficiently process computations on large graphs in systems with read-write asymmetry.

==> biconn.tex <==
\section{Biconnectivity}

In this section we introduce algorithms related to biconnectivity
and 1-edge connectivity queries.
Due to the page limits, here we give an extended abstract of the results while the full version is provided in Appendix~\ref{sec:full-biconn}.

We first review the classic approach, in which the challenge arises since just the output requires $O(m)$ writes.
Then we propose a new BC (biconnected-component) labeling as output, which has size $O(n)$ and can be constructed in $O(n)$ writes.
Queries such as determining bridges,
articulation points, and biconnected components can be answered in
$O(1)$ operations (and no writes) with the \imprep{}.
Finally we show how an \implicit{}
(as generated by Algorithm~\ref{algo:genclusters}) can be integrated into
the algorithm to further reduce the writes to $O(n/\sqrt{\wcost})$.

%All algorithms discussed in this section are easily parallelizable by replacing subroutines by parallel versions.
%The basic algorithm is new and interesting even when interpreted as a sequential algorithm.
%We thus explain the algorithm as a sequential algorithm first, and  later analyze its parallelism in Section~\ref{sec:biconn-depth}.
We begin by explaining sequential algorithms that we believe to be new and interesting.
Then in Section~\ref{sec:abstract-biconn-depth} we show that these algorithms are parallelizable.
For this section, we assume the size of the \local{}
memory in our model is $O(k\log n)$.

In this section we assume that the graph is connected.
If not, we can run the connectivity algorithm and
then run the algorithm on each component.  The results for a graph
are the union of the results of each of its connected components.

\subsection{The Classic Algorithm}

The classic parallel algorithm~\cite{tarjan1985efficient} to compute
biconnected components and bridges of a connected graph is based on
the Euler-tour technique.  The algorithm starts by building a
spanning tree $T$ rooted at some arbitrary vertex. Each vertex is
labeled by $\first(v)$
and $\last(v)$, which are the ranks of $v$'s first and last appearance
on the Euler tour of $T$.
The algorithm also computes $\low(v)$ and $\high(v)$ which indicate the first and last vertex
on the Euler tour that are connected by a nontree edge to the subtree rooted
at $v$.  The $\low(\cdot)$ and $\high(\cdot)$ values
can be computed by a reduce on each vertex followed by a leaffix on
the subtrees.  The computation takes $O(\wcost{}\log n)$ \depth,
$O(m)$ work, and $O(n)$ writes on the \ourmodel\ model, by using the algorithm
and scheduling theorem in~\cite{BBFGGMS16}.  Then a tree edge is a
bridge if and only if the child's $\low$ and $\high$ is inclusively
within the range of $\first$ and $\last$ of the parent.

The standard output of biconnected components~\cite{CLRS,JaJa92}
is an array $B[\cdot]$ with size $m$, where the $i$-th element in $B$
indicates which biconnected component the $i$-th edge belongs to.
Explicitly writing-out $B$ is costly in the asymmetric setting,
especially when $m\gg n$.
We provide an alternative
\imprep{} as output that only requires $O(n)$ writes.
%It essentially constructs an auxiliary graph which is a dual of the vertices and edges of the original graph, and runs connected components on the auxiliary graph.  The cost to just construct the auxiliary graph takes $O(m)$ writes, which can be costly

%\subsection{The \imprep{}}\label{sec:imprep}
\subsection{The BC Labeling}\label{sec:abstract-imprep}

Here we describe the \defn{BC (biconnected-component) labeling},
which effectively represents biconnectivity output in $O(n)$ space.
Instead of storing all edges within each biconnected
component, the \imprep{} stores a component label for each vertex, and a vertex
for each component.  We will later show how to use this representation
along with an implicit decomposition to reduce the writes further.

\begin{definition}[\imprep{}]
  The \imprep{} of a connected graph with respect to a rooted spanning tree
  stores a \defn{vertex label}
  $l:V\backslash \{\textit{root}\}\to [C]$ where $C$ is the number of
  biconnected components in the graph, and a \defn{component head}
  $r:[C]\to V$ of each biconnected component.
\end{definition}

\begin{lemma}
  The \imprep{} of a connected graph can be computed in $O(m)$ operations
  and $O(n + m/\wcost)$ writes on the \seqmodel. Queries about bridges, articulation
  points, or biconnected components can be answered in no writes and $O(1)$ operations
  given a \imprep{} on a rooted spanning tree.
\end{lemma}

%We now describe the algorithm to generate the \imprep{} and the space bound of it, and finally explain how to query on it.
%We ignore duplicate edges in the graph since they do not affect the biconnectivity of the graph.  More specifically, when a tree edge exists, the duplicate non-tree edge is ignored.  Otherwise, only one non-tree edge is considered in the algorithm.   They do affect the checking of bridges, which will be discussed in the query section.

\myparagraph{The algorithm to compute \imprep{}} A vertex $v\in V$ (except for the root) is an articulation point iff there exists at least one child $u$ in the spanning tree that has $\first(v)\le\low(u)$ and $\high(u)\le\last(v)$, and here we name the tree edge between such a pair of vertices to be a \defn{critical edge}.  The algorithm to compute the \imprep{} simply removes all critical edges and runs graph connectivity on all remaining graph edges.
Then the algorithm described in Section~\ref{sec:cc-linear} gives a unique component label that we assign as the vertex label.
For each component, its head is the vertex that is the parent of its cluster in the spanning tree.
Each connected component and its head form a biconnected component.
%The output now is the spanning tree, the labeling of each vertex (indicating the connected/biconnected component), and the articulation point of each biconnected component.

The correctness of the algorithm can be proven by showing the
equivalence of the result of this algorithm and that of the
Tarjan-Vishkin algorithm~\cite{tarjan1985efficient}.

Since the number of biconnected components is at most $n$, the spanning
tree, vertex labels, and component heads require only linear space. Therefore,
 the space requirement of \imprep{} is $O(n)$.

\medskip
Biconnectivity and related 1-edge-connectivity queries on \imprep{} are easy, and we review them in Appendix~\ref{sec:imprep}.

\medskip
The \imprep{} gives the biconnectivity part of Theorem~\ref{thm:main-linear}, which is formally stated as Theorem~\ref{thm:biconn-linear} in Appendix~\ref{sec:full-biconn} (see Section~\ref{sec:abstract-biconn-depth} for \depth\ analysis).

\stepcounter{theorem}\stepcounter{theorem}

\hide{
It is interesting to point out that, the \imprep{} can efficiently answer queries that are non-trivial when using the standard output.
%actually answer more queries that are non-trivial by the standard output.
For example, consider the query: are two vertices in the same biconnected component?  %Namely, is there an articulated point that can disconnect any two given vertices?
With the \imprep{} we can answer the query by finding the label of the lower vertex and checking whether the higher one has the same label or is the component head of this component.  To the best of our knowledge, answering such queries on the standard representation can be hard, unless other information is also kept (e.g.\ a block-cut tree).
}
%Meanwhile, different biconnected components are only connected by articulation points.

%\subsection{The Algorithm with Sublinear Writes}
\subsection{Biconnectivity Oracle in Sublinear Writes}
\label{sec:abstract-bcc-sublinear}

Next we will show how the \implicit{} generated by Algorithm~\ref{algo:genclusters} can be integrated into the biconnectivity algorithm to further reduce writes.
In this section we show the biconnectivity part of Theorem~\ref{thm:main-sublinear} in the case of bounded-degree graphs.  
A more formal result is stated as Theorem~\ref{thm:biconn} in Appendix~\ref{sec:full-biconn}.

The overall idea of the new algorithm is to replace the vertices in the original graph with the clusters generated by Algorithm~\ref{algo:genclusters}.  We generate the \imprep{} on the \clustergraph{} (so the vertex labels are now the \defn{cluster labels}), and then show that a connected-type query can be answered using only the information on the \clustergraph{} and a constant number of associated clusters.
The cost analysis is based on the parameter $k$, and using $k=\sqrt{\wcost{}}$ gives the result in the theorem.

%For simplicity throughout the algorithm description we assume that the graph is bounded-degree.  Later we explain how to relax this restriction.

\mysubsection{The \imprep{} on the \clustergraph}
In the first step of the algorithm we generate the \imprep{} on the \clustergraph{}
with $k=\sqrt{\wcost}$.  We root this spanning tree and name it
the clusters spanning tree.
The head vertex of a cluster is chosen as the \defn{cluster root} for that cluster. (The root cluster does not have a cluster root.)
%The direct successor vertex (the head vertex) of a spanning tree edge
%is named as the \defn{cluster root} for that specific cluster.  (The root cluster does not have a cluster root.)
%For a cluster, we call the \defn{\outver{}} of a cluster tree edge to be the endpoint of this edge outside the cluster.
For a cluster, we call the endpoint of a cluster tree edge outside of the cluster a \defn{\outver{}}.
The \defn{\outvers{}} of a cluster is the set of \outvers{}
of all associated cluster tree edges.  Note that all \outvers{} except
for one are the cluster roots for
neighbor clusters.

\mysubsection{The \localgraph{} of a cluster}
We next define the concept of the \localgraph{} of a cluster, so that each query only needs to look up a constant number of associated \localgraph{s}.
An example of a \localgraph{} is shown in Figure~\ref{fig:localgraph} and a more formal definition is as follows.

\begin{definition}[\localgraph]
The \localgraph{} $G'$ of a cluster is defined as $(V_i \cup V_o,E')$. $V_i$ is the set of vertices in the cluster and $V_o$ is the set of \outvers{}. $E'$ consists of:
%A \localgraph{} of a specific cluster is $G'=(V',E')$, where $V'$ contains all the vertices $V_i$ within the local cluster and the \outvers{} of this cluster $V_o$ (i.e.\ $V'=V_i+V_o$).  Edges in the \localgraph{} include:
\begin{enumerate}
  \item The edges with both endpoints in this cluster and the associated clusters tree edges.
  \item For $c$ neighbor clusters sharing the same cluster label, we find the $c$ corresponding \outvers{} in $V_o$, and connect the vertices with $c-1$ edges.
  \item For an edge $(v_1, v_2)$ with only one endpoint $v_1$ in $V_i$, we find the \outver{} $v_o$ that is connected to $v_2$ on the cluster spanning tree, and create an edge from $v_1$ to $v_o$.
\end{enumerate}
\end{definition}

%An example of a \localgraph{} is shown in Figure~\ref{fig:localgraph}.
Figure~\ref{fig:localgraph} shows an example \localgraph{}.
Solid black lines are edges within the cluster and solid grey lines are cluster tree edges.  Neighbor clusters that share a label are shown with dashed outlines and connected via curved dashed lines.  $e_1$ and $e_2$ are examples of edges with only one endpoint in the cluster, and they are replaced by $e_1'$ and $e_2'$ respectively.

%The input to compute the \localgraph{s} includes the clusters spanning tree and the \imprep{} on the \clustergraph{}.
Computing a \localgraph{s} requires a spanning tree and \imprep{} of the \clustergraph{}.

\begin{lemma}\label{lem:locgraph-cons}
The cost to construct one \localgraph{} is $O(k^2)$ in expectation and $O(k^2\log n)$ \whp{} on the \seqmodel.
\end{lemma}
%\begin{proof}
%Each cluster in the \implicit{} has at most $k$ vertices, so finding the vertices $V_i$ takes $O(ck)$ cost where $c$ is the cost to compute the mapping $\rho(\cdot)$ of a vertex ($O(k)$ in expectation and $O(k\log n)$ \whp{}).  Since each vertex has a constant degree, there will be at most $O(k)$ neighbor clusters, so $|V_o|=O(k)$.   Enumerating and checking the other endpoint of the edges adjacent to $V_i$ takes $O(ck)$ cost.  Finding the new endpoint of an edge in category 3 requires constant cost after an $O(n/k)$ preprocessing of the Euler tour of the cluster spanning tree.  The number of neighbor clusters is $O(k)$ so checking the cluster labels and adding edges costs no more than $O(k)$.
%The overall cost to construct one \localgraph{} is thus $O(k^2)$ in expectation and $O(k^2\log n)$ \whp{}.
%After plugging in $c$ is $O(k)$ in expectation and $O(k\log n)$ \whp{}, the overall cost matches the bounds in the lemma.
%\end{proof}

\mysubsection{Queries}
With the definition of the \localgraph{} and the \imprep{} on the \clustergraph, biconnectivity queries can be answered. Here we take bridges as an example, and the queries for articulation points, \textbf{whether two vertices are biconnected}, \textbf{whether two vertices are 1-edge connected}, and \textbf{biconnected-component labels for edges} are shown in In Appendix~\ref{sec:biconn-sublinear}.
The preprocess steps for the queries are shown in an overview of Algorithm~\ref{algo:biconn}.
With the concepts and lemmas in this section, with a precomputation of $O(nk)$ cost and $O(n/k)$ writes, we can also do a normal query with $O(k^2)$ cost in expectation and $O(k^2\log n)$ \whp{} on \textbf{bridge-block tree}, \textbf{cut-block tree}, and \textbf{1-edge-connected components}.

There are three cases when deciding whether an edge is a bridge: a tree edge in the clusters spanning tree, a cross edge in the clusters spanning tree, or an edge with both endpoints in the same cluster.
Deciding which case to use takes constant operations.

A tree edge is a bridge if and only if it is a bridge of the \clustergraph{}, which we can mark with $O(n/k)$ writes while computing the \imprep{}. A cross edge cannot be a bridge.

For an edge within a cluster, we use the following lemma:
\begin{lemma}\label{lem:bridge-clust}
An edge with both endpoints in one cluster is a bridge if and only if it is a bridge in the \localgraph{} of the the corresponding cluster.
\end{lemma}
%\begin{proof}
%If an edge is a bridge in the original graph it means that there are no edges from the subtree of the lower vertex to the outside except for this edge itself.  By applying the modifications of the edges, this property still holds, which means the edge is still a bridge in the \localgraph{} and vice versa.
%\end{proof}

%Therefore, checking whether in a cluster one or several edges are bridges takes $O(k^2)$ on average and $O(k^2\log n)$ \whp{}.
Checking if an edge in a cluster is a bridge takes $O(k^2)$ on average and $O(k^2\log n)$ \whp{}.
\hide{
\myparagraph{Articulation points}  By a similar argument that a vertex is an articulation point of the original graph if and only if it is an articulation point of the associated \localgraph{}, checking whether articulation points in a cluster costs $O(k^2)$ on average and $O(k^2\log n)$ \whp{}.

%\bigskip
Within this framework, we can also support more query types.
}
\subsection{Parallelizing Biconnectivity Algorithms}\label{sec:abstract-biconn-depth}

The two biconnectivity algorithms discussed in this section are essentially highly parallelizable.
The key algorithmic components include Euler-tour construction, tree contraction, graph connectivity, prefix sum, and preprocessing LCA queries on the spanning tree.
Since the algorithms run each of the components a constant number of times, and the \depth{} of the algorithm is bounded by the \depth{} of graph connectivity, whose bound is provided in Section~\ref{sec:cc} ($O(\wcost^2\log^2 n)$ and $O(\wcost^{3/2}\log^3 n)$ \whp{} respectively when plugging in $\beta$ as $1/\wcost{}$ and $1/\sqrt\wcost{}$).\footnote{The classic parallel algorithms with polylogarithmic depth solve the Euler-tour construction, tree contraction, and prefix sum, since we here only require linear writes (in terms of number of vertices, $O(n)$ and $O(n/k)$ for the two algorithms) for both algorithms.}

For the sublinear-write algorithm, we assume that computations
within a cluster are sequential,
%then each query in a cluster requires $O(k^2)=O(\wcost{})$ expected work and $O(k^2\logn)=O(\wcost{}\log n)$ \whp{}.
and the work is upper bounded by $O(k^2)=O(\wcost{})$ in expectation and $O(k^2\log n)=O(\wcost{}\log n)$ \whp{} for any computations within a cluster.
This term is additive to the overall depth, since after acquiring the spanning tree (forest) of the clusters, we run all computations within the clusters in parallel and then run tree contraction and prefix sums based on the calculated values.
The $O(\wcost{})$ expected work ($O(\wcost{}\log n)$ \whp{}) is also the cost for a single biconnectivity query, and multiple ones can be queried in parallel.
%For most queries we can operate on each cluster in parallel and then run tree contraction and prefix sums based on the calculated values.
\hide{
The exception is for graph connectivity, where the \depth{} to search the neighbor clusters is multiplicative to the \depth{} of the BFS in the low-diameter decomposition.
%The exception is for graph connectivity, where each round of the BFS in the low-diameter decomposition requires querying cluster(s).
Thus the depth of this
algorithm is also bounded by the depth of graph connectivity, which is
$O(\wcost^{3/2}\log^3n)$ \whp{}.
}




==> discussion.tex <==
\section{Discussion on Write-Efficient Connectivity Algorithms}

One may question the necessity of write-efficient connectivity algorithms since it seems that loading the graph to the asymmetric memory requires $O(m)$ space and writes.
While this is true in some applications, it is not always the case.

First of all, there are many applications in which the graph is represented implicitly.
For example the famous Swendsen-Wang algorithm~\cite{swendsen1987nonuniversal} (for studying ferromagnetic phase transitions) is a subgraph of the 2D or 3D mesh in which an edge exists based on local state, and changes from step to step. Each step requires finding connected components. One need not represent the graph explicitly (and most implementations do not).

Secondly, even if the entire graph needs to be stored in the memory, it is still common to define a subgraph using a predicate on edge or vertex labels, and then query (bi)connectivity on the subgraph.
For example, in a typical social network we might query whether two users are connected (via a path).
Connections of interest might be limited to the last week or the last month, or use other vertex/edge availability based on the labels or local information.
On roadmaps we might filter out roads with different conditions and check (bi)connectivity.
%For each such subgraph, our algorithm is run and then (bi)connectivity queries on that subgraph can be answered.
%Running our algorithm and then answering queries on the subgraph can reduce the total work compared to traditional algorithms. 
%Notice that we also introduce a compact representation of connectivity and biconnectivity based on our graph decomposition.
%This indicates that with the same amount of memory space and comparing to classic approaches, we can precompute and store multiple representations (i.e.\ \implicit{s} or \imprep{s}) corresponding to different predicates, while still provide efficiency on queries.
By running our algorithm(s) on different subgraphs and storing our new representations, we can efficiently answer queries for multiple different subgraphs in less space and work than the classic approaches. 

Last but not the least, this paper is concerned with the theoretical question of a tighter upper bound on computing (bi)connectivity under the \seqmodel{} model, whether it is possible to compute (bi)connectivity with a sublinear number of writes, and what the tradeoffs are with respect to extra reads.
We believe this question is of interest beyond the particulars of new memory technologies. 

==> linear.tex <==
\section{Somehow write-efficient parallel algorithms}

\subsection{Connectivity and spanning trees}

Julian and Guy's SPAA paper should construct them using $O(m)$ work, $O(\wcost{}\log n)$ depth, $O(n+m/\wcost)$ writes.



==> morequires.tex <==
\section{Other Biconnectivity Queries}\label{sec:morequires}

We now discuss how some more complex queries can be made.  To start with, we show some definitions and results that are used in the algorithms for queries.

\begin{definition}[root biconnectivity]
We say a vertex $v$ in a cluster $C$'s \localgraph{} is root-biconnected if $v$ and the cluster root have the same vertex label in $C$'s \localgraph{}.
\end{definition}

A root-biconnected vertex $v$ indicate that $v$ can connect to the ancestor clusters without using the cluster root (i.e.\ the cluster root is not an articulation point to cut $v$).  Another interpretation is that, there is no articulation point in cluster $C$ that disconnects $v$ from the \outver{} of the cluster root.

\begin{lemma}
Computing and storing the root biconnectivity of all \outvers{} in all
\localgraph{s} takes $O(nk)$ operations in expectation and $O(n/k)$ writes
on the \seqmodel.
\end{lemma}
The proof is straight-forward.  The cost to construct the \localgraph{s} and compute root biconnectivity is $O(nk)$, and since there are $O(n/k)$ clusters tree edges, storing the results requires $O(n/k)$ writes.

\myparagraph{Querying whether two vertices are biconnected}
Checking whether two vertices $v_1$ and $v_2$ can be disconnected by removing any single vertex in the graph is one of the most commonly-used biconnectivity-style queries.
To answer this query, our goal is to find the tree path between this pair of vertices and check whether there is an articulation point on this path that disconnects them.

The simple case is when $v_1$ and $v_2$ are within the same cluster.
We know that the two vertices are connected by a path via the vertices within the cluster. We can check whether any vertex on the path disconnects these two vertices using their vertex labels.

Otherwise, $v_1$ and $v_2$ are in different clusters $C_1$ and $C_2$.  Assume $C_{\smb{LCA}}$ is the cluster that contains the LCA of $v_1$ and $v_2$ (which can be computed by the LCA of $C_1$ and $C_2$ with constant cost) and $v_{\smb{LCA}}\in C_{\smb{LCA}}$ is the LCA vertex.
The tree path between $v_1$ and $v_2$ is from $v_1$ to $C_1$'s cluster root, and then to the cluster root of the \outver{} of $C_1$'s cluster root, and so on, until reaching $v_{\smb{LCA}}$, and the other half of the path can be constructed symmetrically.  It takes $O(k^2)$ expected cost to check whether any articulation point disconnects the paths in $C_1$, $C_2$ and $C_{\smb{LCA}}$.
For the rest of the clusters, since we have already precomputed and stored the root biconnectivity of all outside vertices, then applying a leafix on the clusters spanning tree computes the cluster containing the articulation point of each cluster root.
Therefore checking whether such an articulation point on the path between $C_1$ and $C_{\smb{LCA}}$ or between $C_2$ and $C_{\smb{LCA}}$ that disconnects $v_1$ and $v_2$ takes $O(1)$ cost.  Therefore checking whether two vertices are biconnected requires $O(k^2)$ cost in expectation and no writes.

\hide{
\begin{enumerate}
  \item if one cluster is the ancestor of the other (WLOG assume $C_1$ is the ancestor and $(v_{C_1},v_{C_3})$ is the cluster tree edge on the path between $C_1$ and $C_2$, $v_{C_1}\in C_1$ and $v_{C_3}\in C_3$), then (1) in $C_1$'s \localgraph{} $v_1$ must be biconnected to $v'$, (2) $v_2$ shares the same vertex label with its cluster root, and (3) $C_2$ and $C_3$ have the same cluster label;
  \item otherwise, both vertices share the same vertex labels with the cluster roots in the \localgraph{s} and the two clusters have the same cluster label.
\end{enumerate}
}

\myparagraph{Querying whether two vertices are 1-edge connected}
This is a similar query comparing to the previous one and the only difference is whether an edge, instead of a vertex, is able to disconnect two vertices.
The query can be answered in a similar way by checking whether a bridge disconnects the two vertices on their spanning tree path, which is related to the two clusters containing the two query vertices and the LCA cluster, and the precomputed information for the clusters on the tree path among these three clusters.
The cost for a query is also $O(k^2)$ operations in expectation and it requires no writes.

\myparagraph{Queries on biconnected-component labels for edges}  We now answer the standard queries~\cite{CLRS,JaJa92} of biconnected components: given an edge, report a unique label that represents the biconnected component this edge belongs to.

We have already described the algorithm to check whether any two vertices are biconnected, so the next step is to assign a unique label of each biconnected components, which requires the following lemma:
\begin{lemma}
A vertex in one cluster is either in a biconnected component that only contains vertices in this cluster, or biconnected with at least one \outver{} of this cluster.
\end{lemma}
\begin{proof}
Assume a vertex $v_1$ in this cluster $C$ is biconnected to another vertex $v_2$ outside the cluster, then let $v_o$ be the \outver{} of $C$ on the spanning tree path between $v_1$ and $v_2$, and $v_1$ is biconnected with $v_o$, which proves the lemma.
\end{proof}

With this lemma, we first compute and store the labels of the biconnected components on the cluster roots, which can be finished with $O(nk)$ expected operations and $O(n/k)$ writes with the \imprep{} on the \clustergraph{} and the the root biconnectivity of \outvers{} on all clusters.
Then for each cluster we count the number of biconnected components completely within this cluster.
Finally we apply a prefix sum on the numbers for the clusters to provide a unique label of each biconnected component in every cluster.
Although not explicitly stored, the vertex labels in each cluster can be regenerated with $O(k^2)$ operations in expectation and $O(k^2\log n)$ operations \whp{}, and a vertex label is either the same as that of an \outver{} which is precomputed, or a relative label within the cluster plus the offset of this cluster.

Similar to the algorithm discussed in Section~\ref{sec:imprep}, when a query comes, the edge can either be a cluster tree edge, a cross edge, or within a cluster.
For the first case the label biconnected component is the precomputed label for the (lower) cluster root.
For the second case we just report the vertex label of an arbitrary endpoint, and similarly for the third case the output is the vertex label of the lower vertex in the cluster.
The cost of a query is $O(k^2)$ in expectation and $O(k^2\log n)$ \whp{}.

\hide{
\bigskip
The preprocess steps for the queries are shown in an overview of Algorithm~\ref{algo:biconn}.
With the concepts and lemmas in this section, with a precomputation of $O(nk)$ cost and $O(n/k)$ writes, we can also do a normal query with $O(k^2)$ cost in expectation and $O(k^2\log n)$ \whp{} on \textbf{bridge-block tree}, \textbf{cut-block tree}, and \textbf{1-edge-connected components}.
}

==> nonconstant.tex <==
\section{Non-bounded degree graphs}\label{sec:nonconstant}

Algorithm~\ref{algo:genclusters}, which generates \implicit{}, and the sublinear-write algorithms on graph connectivity and biconnectivity all require the input graph to have bounded-degree.
This is a strong assumption and in Appendix~\ref{sec:appendix-unbounded} we discussed how to adapt the algorithms to an arbitrary graph.
This construction leads to Theorem~\ref{thm:main-sublinear}.
%in this section we discuss how to relax this constraint to an arbitrary input graph.

\hide{
The challenge of unbounded degree does not affect most of the subroutines in our framework including computing $\rho(\cdot)$, BFS search in connectivity, computing \low{} and \high{} and tree queries in biconnectivity algorithms, etc.
It raises in generating spanning trees either in a cluster (in line~\ref{line:partitionvertex}) to find the partition vertex that cuts of a constant fraction of a tree.

%Thus, as a result of this construction and Theorem~\ref{thm:biconn}, we have the following.

\begin{corollary}
Graph connectivity oracle and biconnectivity queries on a graph can be preprocessed with $O(m\sqrt{\wcost})$ work, $O(m/\sqrt{\wcost})$ writes, and $O(\wcost{}^{3/2}\log^3 n)$ depth on the \ourmodel{} model.  A query also takes $O(\wcost)$ expected operations and $O(\wcost{}\log n)$ \whp{}.
\end{corollary}

This bound using \implicit{} requires less work when $m=O(n\sqrt{\wcost})$.
Otherwise the linear-write version is more efficient on the \ourmodel{} model.
}
\hide{
Here we discuss a solution to generate another graph $G'$ which has bounded degree with $O(m)$ vertices and edges, and the connectivity queries on the original graph $G$ can be answered in $G'$ equivalently.

The overall idea is to build a tree structure with \defn{virtual nodes} for each vertex that has more than a constant degree.
Each virtual node will represent a certain range of the edge list.
Considering a star with all other vertices connecting to a specific vertex $v_1$, we build a binary tree structure with 2 virtual nodes on the first level $v_{1,2\to n/2}$, $v_{1,n/2+1\to n}$, 4 virtual nodes on the second level $v_{1,2\to n/4},\cdots,v_{1,3n/4+1\to n}$ and so on.
We replace the endpoint of an edge from the original graph $G$ with the leaf node in this tree structure that represents the corresponding range with a constant number of edges.
Notice that if both endpoints of an edge have large degrees, then they both have to be redirected.

The simple case is for a sparse graph in which most of the vertices are bounded-degree, and the sum of the degrees for vertices with more than a constant number of edges is $O(n/k)$ (or $O(n/\sqrt{\wcost})$).
In this case we can simply explicitly build a tree structure for the edges of a vertex.

Otherwise, we require the adjacency array of the input graph to have the following property: each edge can query its positions in the edge lists for both endpoints.
Namely, an edge $(u,v)$ knows it is the $i$-th edge in $u$'s edge list and $j$-th edge in $v$'s edge list.
To achieve this, either an extra pointer is stored for each edge, or the edge lists are presorted and the label can be binary searched (this requires $O(\log n)$ work for each edge lookup).
With this information, there exists an implicit graph $G'$ with bounded-degree.
The binary tree structures can be defined such that given an internal tree node, we can find the three neighbors (two neighbors for the root) without explicitly storing the newly added vertices and edges.
Notice that the new graph $G'$ now has $O(m)$ vertices including the virtual ones.
The virtual nodes help to generate \implicit{} and require no writes unless they are selected to be either primary or secondary centers.

Graph connectivity is obviously not affected by this transformation.
It is easy to check that a bridge in the original graph $G$ is also a bridge in the new graph $G'$ and vice versa.
In the biconnectivity algorithm, an edge in $G$ can be split into multiple edges in $G'$, but this will not change the biconnectivity property within a biconnected component, unless the component only contains one bridge edge, which can be checked separately.
}












==> related.tex <==
\subsection{Related Work}

This section will be folded into the flow of the intro...

\paragraph{Asymmetric Memory}
Blelloch et al. defined a theoretical model which takes asymmetric read-write costs into account, and analyzed and designed various sorting algorithms under this model \cite{BFGGS15}. They later designed several other algorithms that do better than their classic counterparts under this model \cite{blelloch2016efficient}. Further work extended their model to a nested parallel setting and offered several write-efficient and work-efficient parallel algorithms \cite{BBFGGMS16}. 
Write-avoiding algorithms \cite{carson2016write} have also been suggested as a form of accounting for the emerging memory asymmetry when designing new algorithms and data structures.

\paragraph{Graph Decompositions}
The clustering subroutine that we introduce is reminiscent of graph decompositions. However, our specifications for the clustering are slightly different from classic graph decompositions. Our only requirement is that the clusters be connected and small; for the purposes of the algorithms that use this clustering as a subroutine, it does not matter if the clusters' diameter is small with respect to their size or whether there are a lot of inter-cluster edges.
In contrast, many graph decomposition algorithms in the literature aim to arrive at a partition of the vertices of a graph into well-connected clusters such that there are few edges that cross between two different clusters. 
%Although graph decomposition provides different guarantees than what we need for our algorithms, it is worth looking at the rich graph decomposition literature to see whether we can gain insights from it.

There has been a lot of work on finding graph decompositions for various applications. The first to suggest graph decomposition was Awerbuch in 1985 \cite{awerbuch1985complexity}. He used them to simulate a synchronous network on an asynchronous one in a distributed setting. Since then, faster algorithms for graph decompositions have been developed.

%In general, a low-diameter graph decomposition is a partition of the vertices of a graph into clusters with low diameter, such that there are few edges that cross between different clusters. 
Recently, a simple and efficient parallel low-diameter decomposition algorithm was developed by Miller et al. \cite{miller2013parallel}. Their algorithm takes a parameter $\beta <1/2$ and builds a decomposition with clusters of diameter $O(\log (n)/ \beta)$ and $\beta m$ crossing edges with high probability, in expected $O(\frac{\log^2 n}{\beta})$ depth and $O(m)$ work. At a high level, each vertex $v$ picks a random delay distributed exponentially with mean $1/\beta$, and then starts building a cluster around itself by executing parallel BFS from $v$. When $v$'s BFS reaches a node that hasn't been reached by someone else yet, that node joins $v$'s cluster. This ensures the required properties. However, we note that this algorithm, even if executed using the write efficient BFS proposed in \cite{BBFGGMS16}, requires at least $O(n)$ writes. Furthermore, while the clusters are guaranteed to have low diameter, there is no guarantee on their size.
\Naama{Probably too much detail on this algorithm}

Many other graph decomposition algorithms have been developed for various different applications \cite{blelloch2014nearly, awerbuch1992low, awerbuch1989network, abraham2012using, linial1991decomposing}. However, none of these algorithms provide us with the necessary conditions to process graphs with a sublinear number of write operations.
%cannot be applied to solve graph problems in sublinear writes either 
% \Naama{There are a few other decomposition algs I've seen, none are applicable; generally, seems like their goals are too different than ours. Should state this better.} 
Further work has considered balanced graph partitioning \cite{andreev2004balanced}, where, given parameters $k, u$, the goal is to find a partition of the vertices into $k$ clusters such that each cluster is of size at most $u \cdot \frac{n}{k}$.
%However, while the diameter of the clusters is guaranteed to be small, their size is not bounded. In our case, when trying to run graph algorithms while keeping the total write cost low, it is important that we ensure the \emph{size} of our clusters is small, and not just the diameter.



==> sublinear.tex <==
\section{Even-more write-efficient parallel algorithms}

\subsection{Connectivity and spanning trees}

Combining previous results should give us an algorithm with $O(m/p)$ work, $O(mp)$ writes, $O((\log n)/p)$ depth.

\subsection{Biconnected components and bridges}

In this section we show how to utilize the \implicit{} to find graph biconnected components (2-vertex connectivity) and bridges (1-edge connectivity) as examples in graph problems.




$q$ offline queries of biconnectivity and 1-edge connectivity can be answered in $O(m/p)$ work, $O(np+q)$ writes on expectation.

Online queries of biconnectivity and 1-edge connectivity can be answered in $O(m/p)$ preprocessing, $O(1/p^2)$ work on expectation or $O(1/{p^2\log n})$ w.h.p.\ per query, and no writes.

Hugely complicated.  Will go back and write more details later.


==> sublinear_decomposition.tex <==

\section{Low Diameter Decomposition with Sublinear Writes}

\newcommand{\clustcenter}{head}
\newcommand{\cluster}{component}
\newcommand{\tentative}[1]{{\color{red} #1}}

In order to design graph algorithms that require a sublinear number of writes, we require a decomposition of the graph such that each \cluster\ of the decomposition is small enough to operate on in the small memory while still having a small enough number of \cluster s. In this section, we present an algorithm for finding such a decomposition. 

The high level idea of the algorithm is to sample points to use as the \clustcenter\ of \cluster s. Points are grouped into \cluster s using a deterministic breadth-first search algorithm. Each \clustcenter\ checks to see if its \cluster\ is too large, and the large \cluster s are partitioned into secondary \cluster s of appropriate size. Upon completion of this step, a graph of the \cluster s is created. The \cluster\ graph can be used to perform computation. Queries can then be answered by having the queried vertex search to its \clustcenter\ to find the appropriate information. 

Our problem is as follows: given a graph $G = \{V, E\}$ where $|V| = n$, $|E| = m$ and some value $k$, find a partitioning of $G$ such that the size of each partition is at most $k$. We have the added complication that the partitioning must take a sublinear number of writes. Our algorithm relies on the assumption that there is a total ordering of the vertices on the graph. We also assume that we have $O(k^2\log{n})$ small memory and that the graph has constant degree. 

The algorithm begins by sampling each vertex with probability $\frac{1}{k}$. Each sampled vertex is treated as the \clustcenter\ of one \cluster. Rather than explicitly assigning each vertex to a \cluster, we have vertices find their \clustcenter\ each time they are queried using a deterministic breadth-first search (BFS). Vertices discovered in the same level of the BFS are searched using the ordering on vertices discussed above. \tentative{Using this search algorithm, a vertex can find its \clustcenter\ in $O(k\log{n})$ time with high probability. }

This sampling methods creates \cluster s with low diameter, but does not preclude the possibility that a large number of vertices end up in the same \cluster. To ensure that no \cluster\ is too large, each \clustcenter\ performs a BFS to find the vertices that are in its \cluster. For every vertex it finds, the \clustcenter\ performs a search from that vertex to see if it points to the \clustcenter. Once the \clustcenter\ finds a vertex that resides in a different \cluster, it can stop searching along that branch of the tree due to the directed ordering of the search. \tentative{Since the degree of the graph is constant and the expected distance from a vertex to its \clustcenter\ is $O(k)$, the number of vertices in a \cluster\ is $O(2^k)$ with high probability. }

As a \clustcenter\ is finding the vertices in its \cluster, it builds a tree representing the \cluster. The root of the tree is the \clustcenter\ of the \cluster, and each vertex is added to the tree such that the path from the vertex to the root consists of the vertices on the path the vertex uses to find its \clustcenter. If this tree is of size at most $k$, then we are done. If the tree is larger than $k$, we can partition it into subtrees of size at most $k$ by counting subtree size and taking a secondary sample at the root of every subtree with size $\geq \frac{k}{2}$. Since every new secondary sample removes at least $\frac{k}{2}$ vertices, the number of secondary samples for a \cluster\ of size $j$ is $O(j/k)$. 

The addition of secondary samples requires a small adjustment to the algorithm a vertex uses to find its center. The search proceeds as described above, except rather than stopping the search upon reaching a secondary sample, that sample is recorded. When a primary sample is found, the path to that vertex on the BFS is checked. If a secondary sample exists on the path, the secondary sample closest to the original vertex is its \clustcenter. 

The result of this algorithm is an implicit construction of a low-diameter decomposition of the input graph $G$. The algorithm requires a sublinear number of writes with only a modest increase in the number of reads. 


